Towards a Deep Multi-layered Dialectal Language Analysis: A Case Study of African-American English

Currently, natural language processing (NLP) models proliferate language discrimination leading to potentially harmful societal impacts as a result of biased outcomes. For example, part-of-speech taggers trained on Mainstream American English (MAE) produce non-interpretable results when applied to African American English (AAE) as a result of language features not seen during training. In this work, we incorporate a human-in-the-loop paradigm to gain a better understanding of AAE speakers' behavior and their language use, and highlight the need for dialectal language inclusivity so that native AAE speakers can extensively interact with NLP systems while reducing feelings of disenfranchisement.

==> 06results.tex <==
\section{Results and Analysis}\label{sec:results}

\subsection{Model Performance Disparity}\label{sec:disparity}

We compare our POS taggers s.t. we can observe each model's performance on the inferred and manually-annotated (Manual) AAE datasets with the intention of examining of fairness issues exist due to a lack of LR data. If so, we attempt to ensure fairness by incorporating LR data in commonly-used off-the-shelf NLP technologies to determine if the inclusion of dialectal languages in these tools contribute to better model performance. 

\begin{table}[ht]
\centering
\scalebox{0.75}{\begin{tabular}{c|c|c}
\hline
\textbf{Tags} & Inferred & Manual\\ \hline
        CC     &  0.73      &    0.95   \\
          CD   &    0.00      &      1.00 \\
          DT   &    0.88      &  0.86     \\
          IN   &    0.81      &  0.79     \\
          JJ   &    0.49      &  0.33     \\
         JJS   &    0.00      &  1.00     \\
          MD   &    0.40      &  0.89     \\
          NN   &    0.67      &  0.71     \\
         NNP   &    0.84      &  0.61     \\
         NNS   &    0.67      &  0.87     \\
         PRP   &    0.97      &  0.92     \\
        PRP\$  &     0.84      & 0.91      \\
          RB  &     0.45     &   0.70    \\
          RBR &     ---     &   0.00  \\
         RBS  &     0.00      &   0.00    \\
          RP  &     0.77      &   0.71    \\
          TO  &     1.00      &  1.00     \\
        UH  &     ---   & 0.72  \\
          VB  &     0.37      &  0.52     \\
         VBD  &     0.56     &   0.43    \\
         VBG  &     0.91      &  0.88    \\
         VBN  &     0.00      &   0.00    \\
         VBP  &     0.43      &  0.46     \\
         VBZ  &     0.80      &  0.62      \\
         WDT  &     ---     &   0.50 \\
          WP  &     0.00      &  0.00      \\
         WRB  &     0.00      &   1.00    \\\hline
\end{tabular}}
\caption{F1 scores of NLTK (Inferred and Manual) POS tag predictions.} \label{tab:tagged}
\end{table}

\begin{table}[ht]
\centering
\scalebox{0.75}{\begin{tabular}{c|c|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Model Performance(\%)}} \\\cline{2-3}
&  Bi-LSTM  & CRF \\ \hline
\textbf{NLTK} & 63.10 & {68.91} \\
\textbf{Manual} & 64.58 & {70.88} \\
\hline
{Diff.} & +1.48 & +1.97 \\
\hline
\end{tabular}}
\caption{POS tag accuracy of the inferred and manually-annotated AAE datasets, and their performance difference.}\label{tab:performance}
\end{table}

In Table~\ref{tab:performance}, we display the accuracy of the inferred and manually-annotated tagged datasets, and their performance difference. As a result of linguistic generalization, we notice that inferred tags, though misclassified also produce similar model performance with little to no explanability. Table~\ref{tab:tagged} displays the F1 scores of NLTK predictioned tags before and after manually-annotated tags showing that models trained under our manually annotated dataset outperform traditional off-the-shelf models in terms of accuracy while maintaining or even improving the prediction performance. Although accuracy margins are relatively small i.e., 1.48\% in the Bi-LSTM network and 1.97\% in the CRF model between the \textbf{NLTK} and \textbf{Manual} AAE datasets, in Figure~\ref{fig:AAE_POS_Tags} we observe that there exist a substantial amount of misclassified tags inferred from the NLTK POS tagger, as a result of non-interpretable linguistic generalizations; this may be due to the differences in language features, default NLTK setting and/or emphatic writing style of authors e.g. ``\textit{Next Wed I Just Wanna Be With Ha n my Baby}'', a sentence consisting of \textit{word-case capitalization}. Word-case capitalization is a writing style that does not comply with the capitalization rules of MAE, thus causing the off-the-shelf NLTK model to assume these words are nouns (see Figure~\ref{fig:AAE_POS_Tags}), and thus, should be lower-cased in preprocessing. 

Tasks such as information extraction and retrieval will fail since commonly used text classification models typically associate content with demographic attributes, thus constituting to a pairwise deficiency of low model performance and language attrition. Unfortunately, these cases may encourage NLP practitioners to continually foster monolingual models to achieve state-of-the-art model performance on downstream tasks using popular ML such as BERT \cite{DBLP:journals/corr/abs-1810-04805}, a well-known deep learning transformer-based model that has been widely used in numerous NLP tasks. However, this notion may continually marginalize LRLs and diglossic communities. Typically, DNNs perform better when given more data; however, this is not the case as our collected and annotated dataset is quite small as it is in a preliminary stage, hence it is not yet adequate to build reliable NLP systems nor derive solid conclusions from it. Consequently, the CRF model achieves higher accuracy. 


\subsection{Syntactic Shifts: Transition Probability}\label{sec:transition}

Within a language, a \textit{syntactic shift} is a form of structural diversity that refers to changes in its grammar; and thus, we propose the question: {{(1) \textit{How do these syntactic shifts constitute to a language's structural diversity?}}} Syntactic shifts enable the author of each tweet, namely, an AAE speaker, to shape a given sequence, and thus highlight structural trends and patterns of AAE's language use given their manually annotated POS tags. 

Let $\mathcal{T}$ represent the number of POS tags in the training data, we use an \texttt{all\_possible\_transitions} function that generates a $\mathcal{T} \times \mathcal{T}$ transition feature matrix. Due to the size of the datasets, we employ this function as it is not computationally expensive. This function generates both positive (likely) {{linguistic}} transitions that occur and negative (unlikely) {{linguistic}} transitions that do not occur in the training data.

\begin{table}[ht]
\centering
\scalebox{0.75}{\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{\textbf{NLTK}} & \multicolumn{2}{c}{\textbf{Manual}} \\
\hline
{Transitions} & {Weight} & {Transitions} & {Weight} \\ \hline
PRP  $\rightarrow$ VBP   &  2.782 & PRP  $\rightarrow$VBP   &  2.010\\
MD$\rightarrow$VB   &   2.284  & JJ  $\rightarrow$NN    &  1.989 \\
JJ $\rightarrow$ NN    &  1.946  & MD $\rightarrow$ VB    &  1.760 \\
NNS $\rightarrow$VBP   &  1.908  & PRP\$ $\rightarrow$ JJ    &  1.722\\
TO  $\rightarrow$ VB  &    1.855  & VBZ $\rightarrow$ JJ   &   1.646\\
\hline
\end{tabular}}
\caption{Top 5 likely AAE {{linguistic}} transitions observed in the CRF model.}\label{tab:likely}
\end{table}

In Table \ref{tab:likely} we show the top 5 likely and linguistic transitions in the CRF model which portray a considerable difference in story telling. By identifying syntactic shifts of inferred tags in comparison to manually-annotated tags we can now examine structural diversity to gain a better understanding of grammatical relations, and hierarchical sentence structures of both \textbf{NLTK} and \textbf{Manual} AAE datasets. We determine that since AAE is close-related to MAE, zero-shot transfer is able to achieve 3 out of the 5 transitions with little explainibility, yet unable to accurately surpass word definitions and word orders to better comprehend context and word ambiguities due to a lack of AAE training data.


 
